Multimodal Image-Text Matching Improves Retrieval-based Chest X-Ray Report Generation

Automated generation of clinically accurate radiology reports can improve patient care. Previous report generation methods that rely on image captioning models often generate incoherent and incorrect text due to their lack of relevant domain knowledge, while retrieval-based attempts frequently retrieve reports that are irrelevant to the input image. In this work, we propose Contrastive X-Ray REport Match (X-REM), a novel retrieval-based radiology report generation module that uses an image-text matching score to measure the similarity of a chest X-ray image and radiology report for report retrieval. We observe that computing the image-text matching score with a language-image model can effectively capture the fine-grained interaction between image and text that is often lost when using cosine similarity. X-REM outperforms multiple prior radiology report generation modules in terms of both natural language and clinical metrics. Human evaluation of the generated reports suggests that X-REM increased the number of zero-error reports and decreased the average error severity compared to the baseline retrieval approach. Our code is available at: https://github.com/rajpurkarlab/X-REM

==> concatenation.tex <==
\textcolor{red}{In the final concatenation layer, we join the possibly multiple output reports of the Natural Language Inference filter into a single document delimited by a space character.  }

==> experiment_intro.tex <==


% We evaluate X-REM on the pre-processed MIMIC-CXR test set and show how X-REM outperforms the prior models across multiple clinical and natural language metrics. Then, we perform a human evaluation of the reports generated by X-REM and the baseline retrieval-based generation model. We also include the results of our ablation studies at the end. 

==> hacks/many-authors-hack.tex <==
% This hack should not be needed anynore as the issue has been fixed upstream in JMLR v1.26 (2020-01-31)
% https://github.com/MIDL-Conference/MIDLLatexTemplate/issues/8
% https://www.dickimaw-books.com/bugtracker.php?action=view&key=141

%\begin{comment}
\makeatletter
% hack the footer of the title page as it doesn't seem to automatically use the et al. version when spanning acros multiple pages
\renewcommand*{\@titlefoot}{\scriptsize\copyright\space\@jmlryear
    \ifanonsubmission
    \space Author(s) names withheld.\hfill
    \else
    \space \@firstauthor\space \emph{et al}.\hfill
    \@reprint
    \fi
  }
\makeatother
%\end{comment}

% \begin{comment}
\makeatletter
% remove the vbox in @jmlrmaketitle which prevents the text to be split across several pages
\renewcommand{\@jmlrmaketitle}{
  % specify the page style in case it spans over several pages. Not sure why this is needed
  \thispagestyle{jmlrtps}%
  % define a new label for the first page as otherwise it starts from 2 in the header
  \label{jmlrstartnew}%
  % hack the spacing to mimick what happens with a vbox
  \null\vspace{-\parindent}\vspace{-2pt}{
  \hsize\textwidth
  \linewidth\hsize
 \jmlrpretitle
  {%
    \def\titletag##1{##1}%
    \@title
  }%
 \jmlrposttitle
 \jmlrpreauthor \@author \jmlrpostauthor
}
% hack the spacing to mimick what happens with a vbox
\vspace{2pt}
}
\makeatother
%\end{comment}

%\begin{comment}
\makeatletter
% hack the footer to use the new counter
\renewcommand*\@jmlrpages{\pageref{jmlrstartnew}--\pageref{jmlrend}}
\makeatother
%\end{comment}

==> method_intro.tex <==
% In this section, we provide a general overview of X-REM. Then, we cover how image-text matching is incorporated in X-REM's report retrieval module and explain the backbone language-image model used to perform image-text matching. We also introduce Cosine Similarity filter and Natural Language Inference Filter which each aims to boost the speed of the retrieval process and the coherency between the multiple reports selected by X-REM. Finally, we go over the learning objectives and the data used for training X-REM.  

==> retrieval_task.tex <==
\vspace{-5pt}

While image-captioning may seem like the natural downstream task for radiology report generation, it has been observed that an image-captioning model often fails to produce a clinically accurate text. The main difference between a regular image-captioning task and radiology report generation is that the latter requires domain-specific knowledge to create a correct report that goes beyond simply spotting the objects present in the image and explains what the noted symptoms may suggest. Moreover, the model's lack of understanding of medical concepts often causes it to hallucinate and generate contradictory statements.  
	
We instead approach radiology report generation as a retrieval task in which the model retrieves, from a corpus of medical reports, texts that best describe the input image. Since the reports in the database were written by experts, their clinical coherency is already guaranteed. Moreover, as there are only a limited number of possible medical descriptions present in the images, a vast retrieval corpus with high expressibility can cover a broad range of symptoms. 

